Quality of Service in Quantum Networks

In the coming years, quantum networks will allow quantum applications to thrive thanks to the new opportunities offered by end-to-end entanglement of qubits on remote hosts via quantum repeaters. On a geographical scale, this will lead to the dawn of the Quantum Internet. While a full-blown deployment is yet to come, the research community is already working on a variety of individual enabling technologies and solutions. In this paper, with the guidance of extensive simulations, we take a broader view and investigate the problems of Quality of Service (QoS) and provisioning in the context of quantum networks, which are very different from their counterparts in classical data networks due to some of their fundamental properties. Our work leads the way towards a new class of studies that will allow the research community to better understand the challenges of quantum networks and their potential commercial exploitation.

==> texcount.tex <==
%TC:macro \myfigeps [ignore,ignore]
%TC:macro \myfigfulleps [ignore,ignore]
%TC:macro \myssec [text,ignore]
%TC:macro \mysec [text,ignore]
%TC:macro \acro [ignore,ignore]
%TC:macro \removed [ignore,ignore]
%TC:group comment 0 0
